Interpolatory Methods for Generic BizJet Gust Load Alleviation Function

The paper's main contribution concerns the use of interpolatory methods to solve end to end industrial control problems involving complex linear dynamical systems. More in details, contributions show how the rational data and function interpolation framework is a pivotal tool (i) to construct (frequency-limited) reduced order dynamical models appropriate for model-based control design and (ii) to accurately discretise controllers in view of on-board computer-limited implementation. These contributions are illustrated along the paper through the design of an active feedback gust load alleviation function, applied on an industrial generic business jet aircraft use-case. The closed-loop validation and performances evaluation are assessed through the use of an industrial dedicated simulator and considering certification objectives. Although application is centred on aircraft applications, the method is not restrictive and can be extended to any linear dynamical systems.

==> figures/algo_discretization.tex <==
\begin{algorithm}[t]
\caption{Loewner-driven discretisation} \label{theAlg}
\begin{algorithmic}[1]
\REQUIRE A continuous-time model $G \in \chinf$, a sampling time $h>0$, an upper bound $\bar{k}$ of the desired order and a number $m$ of interpolation points.
\STATE Sample the interval $]0,\omega_N[$ in $2m$ points $\omega_i$
\STATE Evaluate $R(j\omega_i)^{-1} G(j\omega_i)$
\STATE Apply Loewner to the data-set $\left \lbrace e^{j\omega_i h}, R(j\omega_i)^{-1} G(j\omega_i) \right \rbrace_{i=1}^{2m}$ to get a first model $G_d^m$ that matches all the data and get the underlying minimal order $r$
\STATE Set $k=min(r, \bar{k})$
\STATE Reduce $G_d^m$ to $G_d^k$ as in \eqref{eq:proj}
\STATE Project $G_d^k$ onto a stable subspace, i.e. compute $G_d = P_\infty(G_d^k)$
\RETURN the model $G_d\in\dhinf$ of order $\leq \bar{k}$
\end{algorithmic}
\end{algorithm}


==> figures/systemModelLoad.tex <==
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

% Define a few styles and constants
\tikzstyle{sysProp}  = [draw=white, fill=white,text width=6em,text centered,minimum height=10em,rounded corners]
\tikzstyle{actProp}  = [draw=white, fill=white,text width=4em,text centered,minimum height=2.5em,rounded corners]
\tikzstyle{contPropNom} = [draw=black,thick, fill=green!30,text width=7em,text centered,minimum height=2.5em,rounded corners]
\tikzstyle{contPropAV} = [draw=black,thick, fill=red!30,text width=7em,text centered,minimum height=2.5em,rounded corners]
\tikzstyle{distProp} = [draw=black,thick, fill=green!10,text width=6em,text centered,minimum height=2.5em,rounded corners]
\tikzstyle{ann}      = [above, text width=5em]
\def\blockdist{1.5cm}

\begin{tikzpicture}
    %% SYSTEM
    \node (sys) [sysProp] {};
        \path (sys.0)+(-1cm,0.5cm) node (image) []  {{\includegraphics[width=.4\columnwidth]{figures/7X}}};
    \path (sys.-140)+(-\blockdist,0) node (actuator) [actProp] {Actuator};
    %\draw [->] (actuator.east) -- (sys.-140);
    \path (sys.0)+(\blockdist,0) node (sensor) [actProp] {Sensors};
    %\draw [->] (sys.0) -- (sensor.west);
    
   
    %% INPUT OUTPUT ARROWS
    \path (sensor.0)+(2cm,0) node (outputY) [] {$\y$};
    \draw [->] (sensor.0) -- (outputY);
    \path (sys.-140)+(-4.5cm,0)  node (inputWind) [] {$\u$}; 
    \draw [->] (inputWind) -- (actuator.west);
    \path (sys.140)+(-3.5cm,0)  node (inputAilerons) [] {$\mathbf{w}$};
    \draw [->] (inputAilerons) -- (sys.140);
    
    %% Controller nominal
    \path (sys.south)+(0,-1cm)  node (controller) [contPropNom] {Nominal flight controller};
    \draw [->] (sensor.south) |- (controller.east);
    \draw [->] (controller.west) -| (actuator.south);
    
    %% Controller AV
    \path (controller.south)+(0,-1cm)  node (controllerAV) [contPropNom] {GLA controller $\mathbf K$};
    \path (controller.south)+(-3.5,-1cm)  node (delay) [contPropAV] {$\tau$ delays};

    \draw [->] (outputY.south) |- (controllerAV.east);
    \draw [->] (controllerAV.west) -- (delay.0);
    
    %% Delay
    %\path (controller.south)+(-2,-1cm)  node (delay) [contPropAV] {$\tau$ delays};
    \draw [->] (controllerAV.180) -- (delay.0);
    \draw [->] (delay.180) -| (inputWind);
     
    %% BLOCK ENVELOPPE
    \path (sys.north)+(0,0.6) node (globalModel) {BizJet aircraft $\Htran$};
    \begin{pgfonlayer}{background}
        \path (actuator.west |- globalModel.north)+(-0.2,0.2) node (a) {};
        \path (controller.south -| sensor.east)+(+0.2,-0.2) node (b) {};
        \path [fill=white,rounded corners, draw=white] (a) rectangle (b);
    \end{pgfonlayer}
    
\end{tikzpicture}



